A General Framework for Removing Point Spread Function Additive Systematics in Cosmological Weak Lensing Analysis

Cosmological weak lensing measurements rely on a precise measurement of the shear two-point correlation function (2PCF) along with a deep understanding of systematics that affect it. In this work, we demonstrate a general framework for detecting and modeling the impact of PSF systematics on the cosmic shear 2PCF, and mitigating its impact on cosmological analysis. Our framework can describe leakage and modeling error from all spin-2 quantities contributed by the PSF second and higher moments, rather than just the second moments, using the cross-correlations between galaxy shapes and PSF moments. We interpret null tests using the HSC Year 3 (Y3) catalogs with this formalism, and find that leakage from the spin-2 combination of PSF fourth moments is the leading contributor to additive shear systematics, with total contamination that is an order of magnitude higher than that contributed by PSF second moments alone. We conducted a mock cosmic shear analysis for HSC Y3, and find that, if uncorrected, PSF systematics can bias the cosmological parameters $\Omega_m$ and $S_8$ by $\sim$0.3$\sigma$. The traditional second moment-based model can only correct for a 0.1$\sigma$ bias, leaving the contamination largely uncorrected. We conclude it is necessary to model both PSF second and fourth moment contamination for HSC Y3 cosmic shear analysis. We also reanalyze the HSC Y1 cosmic shear analysis with our updated systematics model, and identify a 0.07$\sigma$ bias on $\Omega_m$ when using the more restricted second moment model from the original analysis. We demonstrate how to self-consistently use the method in both real space and Fourier space, assess shear systematics in tomographic bins, and test for PSF model overfitting.

==> archived_comments.tex <==
% \tianqing{\begin{itemize}
%     \item Weak lensing observation and its increasing challenge in controlling systematics error.
%     \item PSF as a systematics of the weak lensing observable. (multiplicative + additive)
%     \item Previous evidence of PSF higher moments as an additional source of systematics.
%     \item Goal of this paper: build and apply a concise model that include both the second and higher moments of PSF into the weak lensing shear analysis.
% \end{itemize}
% }

%\rachel{I think the intro as written has a lot of the key concepts that are needed.  One that is missing from what I can see is that we are concerned with both {\em PSF leakage in shear estimates} (which is relevant even with a perfect PSF model) and {\em PSF modeling error}.  In most places we are quite vague about the type of systematic we are discussing, and then in a few places we specify modeling error.  I think it's worth being explicit that we are thinking of both -- maybe in the second paragraph?}\tianqing{I have shortly introduced `leakge' and `modeling error' in the second paragraph. }

%\rachel{A second element that might be worth introducing already here is that our framework is based on the idea that we should be considering any spin 2 quantities as potentially generating additive shear contamination.  Right now the wording about the framework is very vague (`a guideline for inspecting and modeling PSF systematics') and I think we should start to introduce key terminology and concepts here in the intro, even if just in a sentence.  You could also explicitly say that we aim to test a complete set of the relevant terms and identify statistically principled ways to downselect to those that matter.  This would basically be making the second-to-last paragraph a crisper articulation of the goals of the paper.}\tianqing{I have added the `spin-2' concept in }

%\rachel{The flow of this section seems a bit strange to me.  At no point to you say what is gravitational lensing or shear, how does it relate to the matter distribution, etc. - it jumps straight to shear estimation (without defining shear, really).  Proposed new structure: before starting 2.1, you have a brief paragraph (with extensive referencing of review articles) defining shear and how it tells us about the matter distribution and cosmological parameters.  Then your `In this section\dots' paragraph can go after.  I then suggest combining 2.1.1 and 2.1.2, as 2.1.2 is very short and conceptually related to 2.1.1.  And then 2.1.3 can stay basically as-is.
%}
%\tianqing{I have added a paragraph in the begining of this section.}

%\rachel{As background, I think it would be worth a paragraph on how the PSF systematics have been modeled in HSC Y1, DES Y3, and KiDS-1000 -- what terms were included?  (all were only second order, but of those, there's leakage, modeling error, and constant -- which were included and what process was used to decide that?  It then sets up the need for the more systematic framework in section 4.} \tianqing{I have added a paragraph in this section that lays out how previous studies model the PSF systematics in their cosmic shear analyses.}

%\rachel{The title is too limiting IMO.  You are developing and demonstrating a general framework for marginalizing over PSF systematics and ensuring the model used is sufficient.  You happen to demonstrate it for HSC - but it's a methods paper of broad applicability.  I would omit HSC from the title and emphasize the generality: `A general framework for removing Point Spread function systematics in cosmological weak lensing analysis'?}\tianqing{That's true. I have changed the title.}

% \xlnt{
% You said that the higher moments are defined in standardized coordinates but you
% are using `$\mathrm{d}x \, \mathrm{d}y$' instead of `$\mathrm{d}u \,
% \mathrm{d}v$' in the equation. I understand that this equation is correct but a
% few steps are missing from your discription to the equation; therefore, readers
% might get confused. Probably, you can note that the determinants of Jacobian
% matrix cancel between the denominator and the nominator.
% }\tianqing{Yes. Fixed}


% Since a spin-2 complex quantity, e.g., cosmic shear, must have rotational
% symmetry at $\phi' = n \pi$,  where $n \in \mathcal{P} (\mathbb{Z})$, the
% polynomial of $x$ and $y$ in polar coordinate ($r,\phi$) must have a angular
% component $e^{2i \phi}$.
% \xlnt{
% This sentence is not mathematically correct since a complex quantity with $n
% \pi$ rotational symmetry can be non-spin-$2$\,. Symmetry under $n \pi$ rotation
% is not a sufficient condition of being spin-$2$\,. Please consider the following
% modification, which is mathematically more accurate:
% }\tianqing{Your suggestion is taken.}





% \xlnt{Am I correct an $r^4$ is missing in the $3$-rd row?}
% \tianqing{Correct, fixed.}


% \xlrv{
% I would suggest using the scalar responsivity $2\,\mathcal{R}$ instead of using
% response matrix here. You can say we assume that there is no spin-$4$ leakage in
% the shear estimation; therefore, we only keep the average of the diagonal
% elements of the responsivity matrix. Moreover, that is consistent with
% definition in equation~\eqref{eq:g}.
% }\tianqing{fixed}

% \xlnt{I think it is better to call $\bar{e}_{\rm gal}$ additive systematics that
% are independent of PSF properties, which can be caused by e.g.\,, optical
% field distortion. That is systematic error as you include it as part of $e_{\rm
% sys}$, but the subscript `gal' is very confusing. Maybe it is better to denote
% it as $e_\text{c}$\,.}\tianqing{That makes sense, fixed.}

% \xlnt{
% You are using $e_\text{c}$ in these equation, which looks good. However, in
% equation~(19) $\bar{e}_\text{gal}$ is used instead. I think $e_\text{c}$ is
% better, and it is better to make it consistent.
% }\tianqing{Fixed.}

   % \rachel{I find the description very confusing.  What do you mean by `full catalog'.  Aren't PSF and non-PSF {\em both} subsets of the full catalog?  And shouldn't all curves be called either `PSF' or `non-PSF'?  Right now it first refers to `PSF' and `non-PSF subset of the full catalog', then it compares non-PSF versus full (for which no curve is shown).}  \tianqing{Fixed.}
    %\rachel{I thought we had concluded PSF and non-PSF stars have different SNR distributions, so how can we say that the widths of the distributions are entirely due to over-fitting?} \tianqing{I have checked PSF and non-PSF at SNR = 300-500, the overfitting still appears. }
    
    
    %\rachel{I'm confused about the statement that it's an overestimate, when the numbers are negative.  Can you say how you've defined the residual, i.e., what is the sign?}\tianqing{This explanation is reworked. }
   % \rachel{Why don't we show the residuals of the moment combinations that matter, instead of the raw moments?  We've done that for 2nd moments, for example -- showing the relevant combinations instead of raw moment residuals.} \rachel{The font in the figure should be a tiny bit larger, to match the paper text.  I suggest removing the Y3 from the legend because that is our default dataset for the entire paper except for one subsection.}\tianqing{Done.}
   
   
   % \xlnt{
%     Did you mention that $e_{c,1}$ and $e_{c,2}$ are two components of spin-$2$
%     quantiy $e_c$\,?
% }
% \tianqing{That's a good point, I have defined them above Eq. 20.}



% \begin{figure}
% \centering
% \includegraphics[width=0.98\columnwidth]{plot/parameter_posterior_nobin.pdf}
% \caption{ The tomographic-free PSF systematic parameter posterior on $[e_{\rm PSF}, \Delta e_{\rm PSF}, M^{\rm (4)}_{\rm PSF}, \Delta M^{\rm (4)}_{\rm PSF}]$, for the fiducial+constant model  catalog(`4+c full'), the fiducial model (`4 full') using the full star, and the fiducial model using non-PSF star catalog (`4+c non-psf'). We see that adding two $e_c$ parameters does not impact the PSF parameter much, therefore can be ignored in the Y3 analysis. Using the non-PSF star, there is significant discrepancy in $\beta^{\rm (2)}$ and $\beta^{\rm (4)}$, which is explained in Section~\ref{sec:res:null}. }
%     \label{fig:delta_xip_redshift}
% \end{figure}





% \tianqing{Regardless of the order and subsections, here are the main results I envision in this paper.
% \begin{itemize}
%     \item In Section III (data), we should put some statistical summary of the Y3 star catalog, something like a scatter of $f_{\Delta \sigma}$ vs. seeing, or some example of PSF higher moments with (ra,dec) in the appendix.
%     \item In the results section, I will include the PSF-PSF correlation functions (in a few panels), the galaxy-PSF correlations without tomography, and how well each model fits the galaxy-PSF correlations. I should also include the plot for galaxy shape constants.
%     \item We should have a plot for the PSF parameter posterior, future cosmic shear analysis can take these posterior as the prior for PSF parameters.
%     \item Need a table for the Likelihood Ratio Test results.
%     \item \textbf{Validation 1:} Switch to redshift bin dependent model and fit it with the galaxy-PSF correlations by tomographic bins. Should have 1 plot for the correlation fitting, and another plot for $\Delta \xi_+(\theta)$, compared to shear-shear signal.
%     \item \textbf{Validation 2:} Compare galaxy-PSF correlation in each field and check if they can be predicted by the corresponding PSF-PSF correlation with the sample PSF parameters. (The assumption here is that the parameters are galaxy property dependent, but are they?)
%     \item \textbf{Cosmology impact (Y1):} re-analyze HSC Y1 shear-shear data vector with the new PSF modeling that include higher moments term. Check the amount of bias on $\Omega_m-S_8$. (one plot) (Use Hamana et al. data vector, covariance, n(z))
%     \item \textbf{Cosmology impact (Y3):} Use redshift-dependent model to apply additive bias to the predicted Y3 shear-shear data vector, and analyze it with gradually simplified models. Check the impact on cosmology again. Use $\Sigma_{y1}/3$ as covariance, data vector from the mock, what about $n(z)$?
% \end{itemize}
% }

%\rachel{Text on plots is too small.  Should be consistent in subscripts: either PSF or psf (right now we mix them).  Should provide some brief high-level takeaway.}\tianqing{Increased Font sizes, added high-level takeaways, homogenize notation for `PSF'.}



%\rachel{I feel this subsubsection did not quite have enough connection to the topic of your paper; it's general rather than motivating the aspects central to PSF systematics models.  I added a couple of sentences to fix that, and put some additional suggestions that, if implemented, should help with this issue. I encourage you to read carefully and look for other opportunities to make this section connect to the modeling you will introduce in the rest of the paper.}\tianqing{Yes, that makes sense. I have added a few more words, mainly to point out the new PSF systematics model is embedded in the forward modeling of the likelihood analysis. }



% I think we don't need to reiterate the potential SNR explanation that we rejected; we can just refer to the section.
    %\rachel{It would be helpful to print the mean $\pm$ error on the mean in each panel (for both PSF and non-PSF), because the bias is small.}\tianqing{That make sense, but I think something more interesting to show is the actual spread of this distribution. Those number give us a tangible sense of how much overfitting is going on. } \rachel{Fair enough; I agree.}
    
%
% Note: text below was way too specific. There are lots of types of null tests besides the ones used here.  I've broadened the text to indicate that these are a specific subset of null tests, rather than being all of the ones that are used in practice.





%\rachel{I'm not sure what this 1-sentence paragraph is doing here -- should it be removed?  Or moved into the intro to the section?  It seems somewhat random and not connected well to the previous or following text.} Null testing provides us a powerful tool to identify and quantify PSF systematics, as well as distinguish between models for the systematics.

%\rachel{Now that you have covariances that are non-negligible for the p-p correlations, does the correlation matrix shown here still substantially drive the results?  Is there any need to show the correlation matrix for the other quantities, perhaps in a different figure or different panel of this figure?}\tianqing{The correlation matrix of the p-p correlation at the best fit parameters of the fiducial model is shown. Also added explanation in the caption and in the text about its impact to the total covariance matrix. }


 %\rachel{Consider making this 1.5 column widths.  It's very hard to see, and quite important.} \tianqing{Increase font size, add high-level takeaway. I think the visibility is okay for this plot now?}
 
 %\rachel{Throughout caption and figure, I think the $e_\text{gal}$ should have hats, for consistency with previous notation?}\tianqing{Fixed.} 
% RM: you fixed the figure; I'm taking care of the caption.


%\rachel{I added the last sentence because those are some key aspects of your method that ensure its general applicability -- and I was afraid that with most of the abstract devoted to HSC Y1/Y3, participants in other surveys might see this as too HSC-specific to be relevant.  That's why I added this, to end on a general aspect of your work. }\tianqing{This looks great, but I am not sure how we accounted for PSF model overfitting in the formalism. The handwavy answer to that would be: ``Well, when there is overfitting, you should use non-PSF stars for the fitting", but in reality we don't have that many non-PSF stars, so we had to do things with PSF stars.} \rachel{Fair enough - I cut it back to `test for'.  It happens to be the case for HSC that we don't have enough non-PSF stars to use them exclusively, but that won't be true for all surveys and analysis setups (e.g., if we were selecting PSF stars self-consistently in all exposures)\dots so I see that as a specific issue for HSC rather than a general issue with the method.  Depending on the severity of the issue one might need to account for it in various ways (e.g., PCA, marginalization with a wide prior, etc.).}\tianqing{Good point, I have addressed this in the future work in the conclusion. }

%\rachel{Some aspects of your method not mentioned here: self-consistent formalism for real space and Fourier space; tests for over-fitting; redshift-dependence; inclusion of a spin-2 constant to absorb 2nd moment biases due to non-PSF factors; and since the number of potential correlations is huge, you have a way of downselecting to the minimal number needed to describe the actual systematics in the data.  I think you should consider briefly alluding to these in the intro.}\tianqing{This is paragraph is now very long, but they are in it now. }


%\rachel{I wouldn't cite Fu et al here, because these results were later recognized to be severely contaminated by systematics issues in the early CFHTLenS studies; I suggest citing the Leauthaud et al COSMOS cosmic shear study and Heymans et al CFHTLenS from around 2013}\tianqing{done}

%\rachel{that's simply the COSMOS survey paper - it's not about redshift estimation or weak lensing - did you mean some other ref?}\tianqing{Changed the citation}

% \rachel{should switch citations here too, as per my suggestions in the intro}\tianqing{Done.}.

%\rachel{It's a bit weird to have a list that just mentions those two, and not Euclid; so you should either mention all three or just mention LSST as an example}\tianqing{Adding Euclid.}


%\rachel{At some point we should probably have one sentence commenting on shear versus reduced shear.}\tianqing{I have put that after Eq.(2).} \rachel{I don't really understand what it means to say reduced shear is `separated from' convergence $\kappa$, can you clarify?}\tianqing{Clarified. I meant `the part of the shear that correspond to the change of the shape'}

%\rachel{I don't understand what this phrase is saying}\tianqing{I have rewrite the sentence.} \rachel{I found this plot quite challenging to comprehend because the lines are so small that it's hard to identify patterns.  Have you considered showing one of the fields with a less extreme aspect ratio?  Or, just showing half of this field, which might reveal trends while still being easy to see?}\tianqing{I have switched to a smaller field: XMM. I think this looks pretty clean to me now. }
    %\rachel{Axis labels: more commonly these are RA and Dec.}\tianqing{Fixed}


% Note: this previously referred to pseudo-$C_\ell$.  However, I would say the formalism and summary statistic is $C_\ell$ and pseudo-$C_\ell$ are simply a measurement method that we use to recover $C_\ell$, hence the edits.
%\rachel{Since part of your paper is meant to provide a formalism for Fourier space, I think it's worth saying `Other work uses Fourier space [CITATIONS] and we will provide the corresponding formalism in this paper.'}\tianqing{Done.} 

%\rachel{Consider citing the Krause et al paper on the likelihood modeling for cosmic shear for DES as a reference one can consult for more detail.}\tianqing{Done} 

%\rachel{Note the terminology change here; we can't call it a `new PSF model' because to most people that will mean that something like PIFF.  Should look for other instances that might need to change.}\tianqing{Noted, I think I at most times call it the  `PSF systematics model', but sometimes I mistakenly call it the `PSF model', which is certainly confusing. I have checked throughout the paper.}

%\rachel{There is a confusing disconnect between this figure and section 4.3.  First, it uses $\sigma$ instead of $T$.  Second, it's not clear what $\Delta M_1^{(4)}$ and $\Delta M_4^{(4)}$ are -- these haven't been defined, we've only defined $M_\text{PSF}^{(4)}$ (and its residual can likewise be presumed to have been defined).  Perhaps it would be more clear to call this the real and imaginary part of $M_\text{PSF}^{(4)}$?  And maybe use similar terminology for second moments?  Or, if not, at least make sure that whatever you use here was actually defined in Section 4.3.  Also, I would suggest putting the two spin-2 components in the left and middle, and spin-0 on the right (or vice versa \dots I just don't see the logic in having the spin-0 in the middle of the spin-2 quantities).}\tianqing{Yes, I have added `PSF' to the subscript. Put the spin-0 components on the left, and show the trace here. } %\rachel{Why are only the non-PSF stars described as subsets of the full catalog?  Aren't the PSF stars also a subset?  It makes the sentence confusing.  I think either both should be described as subsets, or neither one. Otherwise it seems like you are trying to make a point by using that phrase for only one of them.}\tianqing{I think neither is fine. Sorry that was the old description that I didn't found. Checked throughout the paper.}

%\rachel{This terminology is considerably older than those works; what purpose does the citation serve?  The topic of those papers is not so obviously connected to this sentence (e.g., the Eriksen one is about chromatic PSFs).} \tianqing{Changed to some older (and original) references.}  \rachel{The 2001 Bernstein and Jarvis paper uses this phrase, so the ones you've given are definitely not original.  And I'm not even sure that 2001 paper is original.  But if you're going to cite anything as originating this phrase, I would put my bets on that one.  You could alternatively take it as standard terminology that doesn't require referencing.}\tianqing{Yeah, they can be standard terminology.}

%\rachel{One nuance you haven't mentioned here is that in fact HSC measures shear from coadds, as will LSST -- and it's the coadd PSF that matters.  I suggest 1--2 sentences on this, citing our shiny new paper on PSFs of coadded images. This is not merely a gratuitous self-citation; I think the point that coaddition can induce additional issues with PSFs and therefore shear is an important one in the context of this section, and it motivates one aspect of your method: testing at the level of coadds rather than individual exposures.}\tianqing{Yeah, coadd is important for shear estimation. I have put it in the first paragraph as a technical nuance after the `effective PSF'.}

% \rachel{consider refs - same as intro}\tianqing{Add reference here and the intro}.

 %\rachel{$\rho$ statistics do not tell you about PSF size errors and impact on shear calibration, so it cannot justify a choice to neglect multiplicative bias due to PSF size errors.  Were they presumed to have been included within the nuisance $m$ parameter over which they marginalized?}\tianqing{They only neglected the additive bias by the PSF, the multiplicative bias of the PSF is included in the image simulation, so it is calibrated out. I have changed the language in the description here. } \rachel{I don't think so - I thought their simulations had a known PSF, so multiplicative bias due to PSF size errors is not captured by it.  Did I misunderstand their paper?}\tianqing{Ah, right, the multiplicative bias by PSF size was not included in the image simulation. I should say in the begining that we are discussing how previous work treat PSF additive bias. } }

%\rachel{Check out new end of this paragraph, and see what you think.  I think this is important: people will say `I think my dataset might have different systematics and don't want to have to use all these terms', and this is an attempt to preempt that argument.}\tianqing{Thank you, nicely put. }



%\rachel{This section is about more than just the catalogs; it's where you start describing your measurements and results.  I suggest modifying the section title accordingly.}\tianqing{How about `star catalogs for psf systematics correction'?} \rachel{Or maybe `Star catalogs and moments measurements', so it's clear that the measurement process is outlined here?  That's more specific than your suggestion and could be more useful to the reader.}\tianqing{That's a good one, thanks. Done.}


%\rachel{Needs to be updated to eliminate the SNR cut (changes the text and numbers)?  Also should comment on why we think it's OK to relax the cut, after using it in previous papers involving higher moments.}\tianqing{Fixed} \rachel{I think you have to say explicitly that you modify the selection from the previous paper to omit the SNR cut.  Otherwise, it's presumed to be the same (especially since you did call out the other difference in how blending was handled).}\tianqing{Now that we have a new SNR cut, I have updated the entire section.}

 %\rachel{But don't we have {\em some} magnitude cut?  Like the one used for the star catalog in the shape catalog paper?  Otherwise it seems like we would be using all point sources down to the survey limiting magnitude threshold.  Or maybe we use a flag for PSF star candidates?  Either way, there must be some cut that we have failed to mention.}\tianqing{Sorry this is inconsistent from what we do, I have change the text. } \rachel{I suspect the current text is still incomplete.  We know from past work, like Xiangchong's work on the shape catalog validation, that certain flags are needed to get a secure star sample that can be used for PSF tests - e.g., the `extendedness' cut, a lower magnitude cut, and flags that eliminate saturated stars as well.  Surely some of these must be applied here, especially extendedness?  I mean, you say that the SNR>180 cut removes 23\% of the potential non-PSF stars, but that implies there must have been some {\em other} magnitude and flag cuts to make the sample relatively limited in magnitude and SNR range to begin with.  We should outline the flag and other cuts, or point to another paper that does so.}\tianqing{Right, the sample selection is based on the star samples from Xiangchong's shape catalog paper (section 5.1), I briefly mention that and refer the reader to it. }\tianqing{Ah, right, my samples are completely based on the star samples from Xiangchong, so I just refer to that paper for a detailed read. (It is rather complicated to articulate here. )} %\rachel{Need to say why we think it's OK to remove the SNR$>$1000 requirement from previous work on higher moments.}\tianqing{Done}

%\rachel{Say how we chose this.  Was it to make them cover the same range in SNR?  Was it based on empirically checking the size/ellipticity distributions?}\tianqing{Yes, empirical selection based on getting the same size distribution.}

 %\rachel{I feel like we have to explain why, or at least give some potential reasons.}\tianqing{Added the explanation.} 

% \xlnt{
% It seems to me that should be
% $
% \begin{bmatrix} M_{20} & M_{11} \\  M_{11} & M_{02}\end{bmatrix}^{-1}
% $
% in the equation?
% }
% \tianqing{Correct. Fixed}


%\rachel{`mainly follows' implies that it usually follows it, but not always.  I couldn't find any deviations.  If there are some, you should point them out; if there are not, you should delete the word `mainly'}\tianqing{Moment measurements are completely the same, so I deleted `mainly'} 


%\rachel{Do we actually use $\sigma$ later on?  I thought we used the trace.}\tianqing{OK, this is a little confusing, but I will clarify: there are two size defined, trace and $\sigma$. We used trace later for the spin-0 of PSF size, but for the standardization, we have to use $\sigma$ (since we want to move the `Gaussianity' of the PSF, thereby $\sigma$).}

%\rachel{I don't understand the next sentence - can you explain so we can clarify it?  I'm not sure what `the weighted polynomial of $(x,y)$' means.  Do you mean that if you use equation 8 but with the appropriate higher $p$ and $q$ values to determine higher moments, and with the same $\omega$ as before?  If so, you should say that.}\tianqing{That's right, I have changed that. } 

%\rachel{Do you perhaps mean that when you measure the second moments in the {\em image} coordinate system, but use $u^p v^q$ in the integral?  If it's really in the standardized coordinate system then I would think you are measuring $I(u,v)$ rather than $I(x,y)$.  The next sentence also has some issues in how it refers to the coordinate systems; to me, equation 14 is defined in the image coordinate system but using the standardized coordinate system just for picking out moments.}\tianqing{You are right, it's integrating $u^p v^q$, rather than measure the moment in the transformed coordination. I have change the text above Equation 13 to infer that. } 

% \rachel{need to give some pointer describing how we actually use PSFEx for HSC - maybe point to the PDR3 data release paper if it's discussed there, or the year 3 shape catalog paper}\tianqing{Yeah, I should cite the initial description in the HSC pipeline paper, and mention the update in the third data release. }. 

%\rachel{should emphasize here that it's after deblending rather than the original images?}\tianqing{Done.} 


%\rachel{Maybe make this `Spin-2 and Spin-0 PSF moment combinations'?  Since mostly it's combinations of moments that have a well-defined value of spin?}\tianqing{Fixed}


%\rachel{Did we actually show the second part?  We definitely showed the first part.  It seems to me that we simply {\em assume} the second part, in the very next paragraph.}\tianqing{Yeah, I think throughout the paper we assumed that spin-2 couple with spin-2, which is understandable, but also better to be clear.}  \rachel{To connect back to your (a), don't we also have to comment on the fact that odd order moments have no spin-2 combination?  If so, we should say that here.  I suggest wholesale moving your sentence saying `In Appendix~\ref{sec:ap:spin2}, we prove that only the even moments can combine and compose spin-$2$ moments.' here and explicitly connecting it to (a).  This makes more sense than randomly jumping to it in a paragraph that is mostly talking about 6th moments. }\tianqing{Yes, that makes sense. I moved that sentence here and taped them together. }\tianqing{I changed the title of this section to `spin-2 and spin-0 PSF moments', rather than `spin-2 higher moments'.}

%\rachel{I think this paragraph will seem better motivated if the sentence about even moments providing spin-2 quantities moves earlier, as I suggested.  You could then refer to it briefly and say that that finding suggests we may not be able to stop at 4th moments, or at least need to test whether that's OK.}\tianqing{I agree, I added a sentense in the begining of this paragraph saying even higher order can generate spin-2 moments, for example, 6th moments...} 


%\rachel{Can we really state this so generally?  Or can we only say this is true for our HSC catalog?  This is important, because if it's a result specific to this catalog then we need to say we have demonstrated this here but we recommend carrying out this test routinely in order to define the complete set of spin-2 quantities any survey should care about.}\tianqing{No we can't. I should say this is HSC specific because our 6th moments are highly correlated to fourth moments, and are noise dominated. }



%\rachel{I think the logic and narrative here need some help.  Currently we go from spin-2 4th moments to spin-0 2nd and 4th to spin-2 6th moments, so we're bouncing around from spin-0 to spin-2 to spin-0 and from moderate to low to high order, in a way that is kind of jarring and not well explained.  Can this be improved -- either improve the order or better explain the logic?}\tianqing{I have re-arranged this section: first describe spin-2 (both fourth and sixth moments), show the spin-2 whisker plot, then spin-0, then show the distribution of both spin-2 and spin-0.}

%\tqchange{\rachel{This paragraph is an example of what I mean re: logic.  The section is about spin-2 quantities and we haven't said why we should care about spin-0.  I think an appropriate intro to this paragraph would be to say that while it's the spin-2 quantities that affect shear, you can get spin-2 directly or as spin-0 times spin-2, so let's figure out what spin-0 quantities are relevant (and could also point to the Jarvis et al paper with the extended $\rho$ stats including the PSF trace in support of this idea).}\tianqing{Improved the introductory paragraph, and added some sentences here is link up the logic. } 


% RM: this paragraph seems unnecessary to me - we don't need to give all these details when section 5.1 will just give them again.  To compensate for commenting it out, I've slightly elaborated the sentence about section 5.1.
%In this section, we introduce the method of modeling the leakage and modeling error of the PSF systematics, including both second and higher spin-2 quantity in the cosmic shear analysis. In addition, we consider adding a mean ellipticity to the systematics model.
% \xlnt{I think you also model constant additive bias that is independent of PSF
% property. Sightly mention it here is better.}\done

    %\rachel{Need to comment on errorbars: how did you calculate them?  Why do
    %some curves seem to have them and others not --- is it that they are too
    %small to see on some curves?}
    %\rachel{The middle panel has two colors that look extremely similar to me
    %(I can't tell the two oranges apart).  Can you choose something else from
    %the color palette, or use black for one of them?}
    %\tianqing{Commented on errorbars, Changed on colors. }

 %\rachel{Do you want to reiterate here that it is specifically the spin-2 quantities related to the PSF that contribute here to $e_\text{sys}$?}\tianqing{Done.}


%\rachel{I thought here we were just trying to present our framework in a generally applicable way.  But the text after this seems specific to HSC shear inference, re-Gauss, etc.  Need to work on that -- make it general but comment on HSC-specific aspects as examples we use to illustrate the method.}\tianqing{I agree, done. } 

%\rachel{We should comment on why we end the model there.  How do we know there aren't other terms?  Should point, again, to appendix that we use to motivate this and emphasize our general approach involving all spin-2 moment combinations.}\tianqing{Done.}

% \xlnt{$\mt{R}^2$ is very confusing and I think that is not a correct notation
% since $\mt{R}$ is a matrix. If we change that to $2\mathcal{R}$, it will be much
% simple to understand.}\tianqing{Fixed}

%\rachel{I think the notation could be confusing: the first is a set of numbers that we think, in practice, are defined for the ensemble (not each galaxy or each galaxy position).  The second is a set of a numbers that we think has a different value at each position on the sky.  Maybe point this out explicitly so we are up front about what each quantity really means?}\tianqing{Done.}

%\rachel{It's confusing that the summation goes from 1 to 4, but the length of $\ve{p}$ is actually 6 as you defined it in the text, and it includes the constant terms like $e_{\text{c},1}$. Given that the constant terms have to be called out separately, shouldn't we just leave them out of $\ve{p}$ so that $\ve{p}$ and $\ve{S}$ have the same length?  I guess you've kept them in so that they are implicitly included in your log-likelihood, so if you want to keep them there, you might want to just explain why (given that it looks rather strange here).}\tianqing{Yeah, the reason that $e_c$ is there is to include them in the parameter vector in the likelihood inference equations. I have explicitly mentioned why $e_c$ is included, and also explicitly mention that the summation is over the first 4 terms. }

%\rachel{I think the terminology here re: average shape is very confusing.  Any catalog can have a nonzero mean shape due to cosmic variance, and this effect can be quite significant even for decent-sized fields.  But that's not a systematic and it's not what we refer to with $e_c$.  I suggest that when defining $e_c$ you explicitly say that this is meant to encapsulate any {\em other} systematic that can cause a non-zero mean shear, which cannot simply be estimated by finding the mean galaxy shape across the catalog, due to cosmic variance.  And then be very careful to fix this and any other instances of `average shape' to refer to the constant systematics term instead.  (The average shape is something different - we measure it in order to quantify systematics but it has non-systematics contributions.)}\tianqing{Yes, I have added an extra explanation when we define the constant systematics term. And change the other places mentioning `mean shape', and `average shape', to mention that this term is the `constant systeamtics'.}

%\rachel{Nominally the first summation has 16 terms, but you refer to 10.  Perhaps you should say that only 10 are unique?}\tianqing{Yes, fixed.} 

%\rachel{Traditionally `null tests' are used just to test if there is a problem of some sort.  But that isn't what you are doing here.  You are using them to build a model for the PSF systematics and impact on WL shear, over which one can marginalize.  I'm afraid the section title is deceptive and may suggest to people you are doing something far simpler than that.  Have you considered renaming it to better reflect what's happening in this section?  For example, `Building a data-driven systematics model'?  That's basically what you are doing, using the formalism in 5.1.}

%\rachel{This subsection is long and fairly complex.  I suggest either breaking it into subsections or subsubsections.  For example, you could have one for the basic fitting process, one for use of PSF vs.\ non-PSF stars, and one for cosmological impact.}


    %\rachel{This caption is confusing in a few ways.  First, I think the left panel has equations 25 and 27, not 25 and 26 as the caption says; similarly, the right panel has 26 and 28, not 27 and 28.  Second, I think it's deceptive to refer to these as `Leakage' and `Modeling error'.  For example, in practice, $\langle \hat{e}_\text{gal}e_\text{PSF}\rangle$ can have contributions from both leakage and modeling error, and even from the constant systematics term.  I suggest rewriting this first sentence accordingly, and changing the plot titles.  Perhaps you could call these `Correlations with PSF quantities' and `Correlations with PSF model residuals' (in the caption and title) or something like that?}\tianqing{Fixed the label, and title. }

%\rachel{looks like it's also true for fit-second?}\tianqing{Yes, fixed.} %\rachel{Why do you need the `*$e_\text{PSF}$' and so on at all?  Can't you say that the color is used to show what is being modeled?  That is always true except for `fit second'.  So if you change `fit second' to match what you are modeling, then you can simplify both legends considerably.}\tianqing{Fixed} 


%\rachel{In the legend, it looks like you've used $<>$ rather than $\langle\rangle$ (inequality symbols rather than angle brackets)?}\tianqing{Fixed} %\rachel{Font in text on the plot is too small.  These plots are critical; have you considered letting them take more space, for example have the first two together and then put the third into a separate plot?  Currently it's hard to distinguish the smaller symbols for the points without zooming in.}\tianqing{Increased font sizes, homogenized to ``PSF'' (figures and text), moved the third panel to a separate plot.}


% \rachel{this notation differs from the axis labels; should make them consistent.  Also have you considered using $\langle\rangle$ to indicate it's an ensemble average?}\tianqing{Yes, it's not that consistent. I will switch to `$\langle \hat{e}_{\rm gal} \rangle$'} \rachel{OK, but have to do that in the plot axis labels too so they are consistent}\tianqing{Fixed}


%\rachel{I don't really understand this -- I thought the `2' and `4' models do not have any $e_c$ term, and only the models with `+c' have it.  So why are there 4 model points?  I thought there should be two.}  \tianqing{`4' and `2' do not have $e_c$ term, but they also predict $\langle e_{\rm gal} \rangle$ by the first 4(2) terms in Eq.~\ref{eq:null_ave}. So as long as the best-fit value for $\langle e_{\rm gal} \rangle$ is within 1$\sigma$ of the data, then the model is sufficient.} \rachel{Oh - I think the issue here is that the sentence I commented on is wrong?  It says you've plotted the best-fit $e_c$, and those models do not have $e_c$ -- but it sounds like you're actually plotting the best-fitting $\langle e_{\text{gal},i}\rangle$ values from equation 29 including all model contributions?  If so, then that sentence needs to be fixed to say what is plotted (and maybe point to equation 29) and then it's all good.}\tianqing{Yes. Fixed.}


%Null tests are used to estimate contamination from systematics in the
%shear catalog.  One type of null test involves cross-correlating the galaxy shears with unrelated
%physical quantities, e.g.,  cross-correlating shear and PSF moments. The
%correlation is supposed to be zero if there is no contamination, hence the name
%``null test''.  

%\rachel{need to call back to constant term as well}\tianqing{Yes, the constant is mentioned at the end of the paragraph} \rachel{No, I'm not referring to the measured quantity $\langle \hat{e}_\text{gal}\rangle$.  I'm referring to the fact that $e_c$ directly contributes to the cross-correlations you are discussing here.  In other words, you wrote that the g-p cross-correlations depend on PSF 2nd and 4th moments, but really they depend on PSF 2nd and 4th moments and $e_c$ as shown in the equations 26-29 (this section can't ignore it because it's part of the overall model we present)}\tianqing{I see, that's right. This section cannot ignore the constant systematics term.}.  



%\rachel{Should the transpose be on the first term, not the third?  I don't think the math works if it's on the 3rd.}\tianqing{Yes, if the vector is a row vector.}
% The vector is a column vector -- it has dimensions N x 1.  So if you put the transpose on the first one, then you get (1 x N) x (N x N) x (N x 1) which is a valid multiplication giving a scalar.

%\rachel{Say what MCMC method/code was used.}\tianqing{Done}

% \tqchange{Note that here we only consider the uncertainty on the g-p correlations, and neglect that of the p-p correlation.  To justify this choice, we conducted the following test: We inferred the posterior of $\ve{p}$ by stacking the posterior from 20 samples drawn from the p-p correlation distribution of the non-PSF stars. \rachel{This sentence was too vague for me to understand what was done.  20 samples of what?  What is the `p-p correlation distribution'?} The resulting $\ve{p}$ uncertainties only increased by at most $5\%$, justifying our choice to neglect the uncertainty on the p-p correlation. }
% \tianqing{Specify how we marginalize over p-p correlation uncertainties.}

 %\rachel{Have you shown this?  I would think you have two options, one being fit-second and one fit-second-plus-constant, and you'd have to do a statistical test to confirm which is the model of choice.  If you did that, you should mention it; but if you didn't do that, then I think this sentence needs to be softened.}\tianqing{I didn't do a fit-second+constant, so I softened the sentence. }  

% Note: changed from `selection' to `comparison' because we opt not to select a model based on $p$-values or AIC alone.

% Note: 2+c is also a 4-parameter model but doesn't work, so I changed it to `include fourth moments explicitly.

 %\rachel{spell out acronym and give citation}\tianqing{Done.} 

 %\rachel{Correct me if I am wrong, but I think you cannot compare their AIC values with anything (they are distinct datasets and models).  For that reason, I'd deliberately omit their AIC from the table, to avoid giving the impression that we can do anything meaningful with it (and say why it's omitted in the caption).}\tianqing{Yeah, that make sense. I took out the AIC of the non-PSF stars and fit-second for the PSF stars. }
% RM: I updated the caption to reflect this choice.

 %\rachel{Text is too small.  Also, in previous plots like figure 1, your PSF vs non-PSF color scheme differed; should homogenize.}\tianqing{Increased font size, homogenized color.}


%\rachel{Say what is the vertical line.} \tianqing{They are just the grid lines, I changed them to dotted lines, so that they are not that obviuos.} \rachel{It's true that the `up to an order of magnitude' is the most relevant point when comparing models.  But I think it's also relevant that the contamination is now exceeding 10\% of the signal in the lowest bin, meaning the contamination is now relatively more important.  Should probably point this out.} \tianqing{Done.}

 %\rachel{This is the first time the phrase `fiducial cosmology' has appeared.  Consider pointing to the table where it is defined?}\tianqing{Done}



%\rachel{I suggest pointing to the section where the models are defined, so people can go read about it.  I also suggest explicitly commenting on the models enough that the big picture emerges from the caption: for example, I suggest flagging that `4+c' is a parent model and all but fit-second are sub-models, and that `4' is considered fiducial based on what's in the table.}\tianqing{Done.}
%\tianqing{I agree, I have removed the AIC of the fit-second and the non-PSF stars. }  %\rachel{I'm worried the presentation of fit-second in this table will result in numbers being misused.  In particular, it's not clear from the table that this model is fit to a different set of data or that its AIC should not be compared with the others.  My suggestion is that you work on a way to indicate it's fit to a different set of data, and actually {\em omit} AIC (it's only for model comparison and you cannot compare this model with the others), and say why.} 

%\rachel{Like previous plots, need to modify the caption and figures: these aren't purely leakage and modeling error, but rather correlations with PSF shapes and shape residuals.}\tianqing{Fixed} 


%\rachel{This is confusing: it seems like there should be two sets of data points and two model curves on each plot.  But the legend only seems to show the data points?  And there are shaded regions around the points that aren't described, and grey shaded regions that are also not described.}\tianqing{Fixed}  %\rachel{text too small; this is true for most plots so I will stop writing it in all captions} \rachel{Not sure you need to repeat identical legends in top and bottom rows} \rachel{I would suggest including any multiplicative factors in axis labels rather tahn as tiny numbers up top -- i.e., call the top row $10^5 \xi$ in the y axis, rather than $\xi$ with a little $10^{-5}$ on top of the axis.  Same comment applies to other figures.}\tianqing{Increased fonts, and get rid of repeating legends. Also put multiplicative factor into the axis labels. }

%\rachel{psf versus PSF subscripts?}\tianqing{Fixed} 

%\tianqing{Increased fontsize, add high-level takeaway.} 

%\rachel{I think it'd be useful to show the marginalized posteriors for the redshift-independent model also (one additional curve in each panel), so we can see whether it looks like an average or is it more complex.}\tianqing{Done.} 


%\rachel{I don't see black circles, and the legend only shows the triangles.  Also, what is solid vs.\ dashed line?  It doesn't seem indicated in the caption or legend, but it seems potentially important.}\tianqing{Added the z-ind. (non-PSF) into the legend and caption.}  

%\rachel{Figure only seems to show one set of black points from what I can see (and as indicated in the legend); is this out of date?  To be honest, I worry it would be trying to do too much if we show the z-independent vs.\ z-dependent model and PSF vs.\ non-PSF.}\tianqing{I made some tiny change to improve the visibility: use different capsize for the PSF and non-PSF errorbar, decrease the transparancy of the black data points. I think breaking up this plot is also very hard, since we want to compare the PSF vs. non-PSF, and z-dependent vs. z-independent at the same time. (There are 4 sets of comparison.)}  

%\rachel{I'm not sure how to see this from the plot?}\tianqing{I slightly edited the conclusion here.} 

%\rachel{The previous sentence doesn't mention redshift at all, and implies the focus of the figure is PSF vs.\ non-PSF stars; need to rethink this presentation.}\tianqing{I included all the models shown in the plot.} 

%\rachel{Likewise\dots}\tianqing{I hope it is a bit clearer now. }

%\rachel{Need to say to what degree these choices are in agreement with those of Hamana et al.}\done 




%\tianqing{Need a suggestion for Y3 analysis, but I am still debating. } 
%\rachel{I think this could be covered by what we discussed today: AIC has a weak preference for redshift-dependent modeling, but the redshift-independent model can adequately describe the data.  Since we don't want to have four parameters, we'll check/confirm in section 6 that it doesn't induce unacceptable cosmological parameter biases, and (spoiler) it doesn't, so that is our recommended model for Y3.}
%\tianqing{This makes sense, I have defer the decision making to Section~6.} 

%\rachel{Incidentally, I think it's overly simplistic to suggest that the choices are 4 vs.\ 16 for redshift-independent vs.\ redshift-dependent.  It would be completely fair to look at figure 11 and say the main impact of redshift evolution is to induce some power-law dependence of $\beta^{(2)}$ on $1+z$, so you give $\beta^{(2)}$ such a power law and keep the others fixed.  That covers the most statistically significant trend and is only a 5-parameter model (or 4 if you fix the power law index based on what you find in figure 11).  I think we do need to acknowledge this possibility of parametrized redshift dependence with few additional parameters, though it's a question of whether that's just some words or an actual test that you do in section 6.}
%\tianqing{Thanks, I added some discussion at the end of the section.}

%\rachel{Should say what is the vertical line and shaded region in the bottom, and the shaded regions in the top panel.}\tianqing{Done.} %\rachel{This would be easier to see if you had a bottom panel that showed the $S_8$ and $\Omega_m$ constraints for the 3 cases as a horizontal line with errorbars (easier to see $0.2\sigma$ shifts).  Same comment applies to next figure.} \tianqing{I have added the 1-d contour}


%Additionally, the errorbars on $\Omega_m$ shrink by $11\%$ compared to the no correction. \rachel{And they get larger for $S_8$.  I'm not sure this is particularly important to report, since it just represents tradeoffs in errors between two parameters that we care about, and the biases are the more important part.} \tianqing{Yeah, it's hard to tell. I will delete this comment.}
% The $\Delta \chi^2$ between the second moment model and no correction is $3.3\pm0.4$, but the $\Delta \chi^2$ between the fiducial model and no correction is a whopping $16.6\pm 0.4$. This means with only 2 extra parameters, the fiducial model is able to improve the model fitting of HSC Y1. 


% Assuming an effective degree-of-freedom $170-3 = 167$, the $p$-value of the analysis with the fiducial model is 0.53, compared to the $p$-value of 0.30 for the analysis with no correction. These results provide evidence that with our new PSF systematics model, the theoretical model is able to better fit the Y1 cosmic shear data vector.


%\rachel{should comment here on the offset from the input -- how should that be interpreted, and comment on the solid vertical line as well}\tianqing{Done} 

%\rachel{Not clear what this means - are you saying you actually don't use the ones from Rau et al as was stated above?  Should the earlier sentence instead say `estimated in an early version of Rau et al.'  instead, so that it's clear the change is from a pre-submission version to a more recent one?}\tianqing{Yes, it's an earlier version, I have edited the sentence. }  \rachel{It is also the case that scale cuts, covariances, and potentially some modeling choices will differ in Y3.  Should mention this too.}\tianqing{Done}


%\rachel{I'm not sure about this.  It overshoots in one dimension ($\Omega_m$) and undershoots in another ($S_8$) so I don't think we can say it overshoots the true contour?  At most we could say it overcorrects $\Omega_m$ and under corrects $S_8$, I think.}\tianqing{Fixed} 

%\rachel{Should this last sentence be talking about the {\em uncertainty} on $S_8$, to be parallel with the previous sentence which was about the uncertainty on $\Omega_m$?  Right now they aren't parallel - we talk about impact on the uncertainty on $\Omega_m$ and impact on $S_8$}\tianqing{I rewrote this paragraph, the previous one is really disoriented. } 

%\rachel{Is there a reason to focus here on $\Omega_m$?  The best-constrained parameter direction is $S_8$ so may be of more interest.}\tianqing{I have added the results on $S_8$.}

% \tianqing{I should add a paragraph to conclude the model selection inferred by the results here.}


%\rachel{At some point, I think it would be good to insert a concise summary of the method.  Currently section 5-6 mix method description and results in a way that makes a clear narrative, but for somebody who doesn't work on HSC, they would probably want to see a short enumerated list of steps without all the intervening `here's what happened when we did this in HSC'.  Maybe it could be a short section, located here, called `Method summary'.}\tianqing{Here it is.}

 %\rachel{Here would be a good place to say something like `The overall outline of our method is summarized in Section ??.' - that's a nice reminder before diving into the results of applying it to HSC.}\tianqing{Done.} 



% \rachel{I'm a little confused about this paragraph.  We already said earlier in the conclusions that we recommend a fiducial model with 2nd and 4th moment terms.  So should this justification be merged into that earlier text?  Or should it just be removed or condensed to focus on the recommendation for future surveys?  It seems duplicative, and it especially doesn't make sense to me that it goes after the paragraph about small effects that don't matter. }\tianqing{Yes, the beginning is duplicative. I just move the motivation to the future surveys to the future work paragraph. }
% We show that in the HSC Y3 catalog, the PSF fourth moment leakage is a leading contributor to the PSF additive contamination to shear.  This effect is captured by our fiducial model, but not captured by the second moments-only model which has been used for past analyses. This means that the second moments-only model will fail to correct most of the PSF contamination in shear. These results drive our recommendation that the HSC Y3 cosmic shear and joint-probe analyses use a PSF systematics model that considers fourth moment leakage and modeling error. 

% \tianqing{To do list:
% \begin{itemize}
%     \item remove double citation
% \end{itemize}
% }

% \rachel{I know I advocated for a general title, but I think this one might need work: we aren't providing a framework for all (multiplicative and additive) PSF systematics.  How about inserting the word `Additive' in the title?} \tianqing{That makes sense. Done}

%\rachel{This last sentence is a statement about the covariances, but nothing is said about the correlation matrix that you've shown.  Is there anything useful to say here about what you've shown in the plot?  Also, it's notably quite noisy and might be worth mentioning that the top comes from many mocks while the bottom comes from jackknife, to explain that.}\tianqing{I have added an explanation for the noise, and the high correlation across angular bins. }

%\rachel{Figures in this section seem out of order; once the text settles, should rearrange the figures accordingly.}\tianqing{I think the order is correct now. }


%\rachel{I think it would be helpful to move $e_c$ out of the correlation, as a reminder that it's just a spin-2 number rather than a spatially varying quantity.}\done

 %\rachel{Justification of this choice?}\tianqing{I am not sure if the justification makes sense.} 

 %\rachel{I don't follow the logic in the previous sentence; can we discuss and try to clarify?}\tianqing{The PSF star underestimated $\Delta e_{\rm PSF}$ and $\Delta M_{\rm PSF}^{\rm (4)}$ by a factor of roughly 2. Therefore, for the model to compensate, $\beta^{\rm (2)}$ and $\beta^{\rm (4)}$ would be overestimated by a factor of 2. Does this sounds logical?} \rachel{No, I still don't understand.  It seems to come with an assumption that the systematics terms must be the same as estimated by PSF and non-PSF stars, and I don't understand where that assumption comes from.  It seems to me that one of them could just be wrong, in which you can't talk about compensation.}\tianqing{Yeah, for the PSF stars, both $\Delta e_{\rm PSF}$ and $\beta^{\rm (2)}$ are wrong, but the $\Delta e_{\rm gal}$ is still correct, because the model is fitted to $\Delta e_{\rm gal}$. Maybe I am not clear enough in the text, but that's what I meant by `$\Delta e_{\rm PSF}$ is underestimated by  a factor of 2, and $\beta^{\rm (2)}$ is overestimated by 2'.}
% I spelled it out some more.

%\rachel{Do we, at some place in the text, say where these values and priors come from?  I can't find it, and I think we should be saying that.}\tianqing{I added that to Section~6.2.}

%\rachel{I'm not quite sure what is meant by saying you adapted a cosmological model?}\tianqing{Yeah, it doesn't make sense, we can just say we build the cosmological model in cosmosis.}


%\rachel{One obvious question is how did you validate this model, why do we believe it's relevant, etc.  Perhaps this could be addressed by qualitatively commenting on how well your constraints with the `fit-second' model match those of Hamana et al.?  That's not the main point of the paper, but it certainly seems relevant to the validity of the new analysis code and the setup you've described here. }\tianqing{I have added a paragraph for comparing our results to the Hamana et al. results. }


% \rachel{At some point it is probably worth doing an AIC comparison, to see if AIC thinks the additional params are worthwhile.}\tianqing{Done.}

%\rachel{There is a well-defined formalism to determine the effective degrees of freedom in a fit (accounting for prior-dominated parameters): https://arxiv.org/abs/1806.04649  We might want to use that rather than the naive calculation here.  But that is less important and can wait until the paper is being reviewed by the WG, I think.}\tianqing{I think a way to deal with this is just ignore the absolute $\chi^2$, rather, discuss the $\Delta \chi^2$, which is more useful in terms of modeling comparison. } \rachel{No, that doesn't help, because the effective difference in the number of degrees of freedom to use when providing a statistical interpretation of $\Delta\chi^2$ is also affected by this issue.  And I think we really want to use $\chi^2$ sometimes, for example, to answer the question of `is this model an acceptable fit' (even if not the best).  Xiangchong definitely has implemented this calculation and my understanding is it should be easy to carry out with the info you have, so I suggest talking with him.}\tianqing{Switched to using $\chi^2$ and effective degree of freedom.}


% \rachel{Are you sure those aren't the $n_{\rm eff}$ values, rather than $170-n_{\rm eff}$?  That's what it looks like to me.} 

%\rachel{Show the right answer on this plot, since it's a mock.}\done

 %\rachel{I see this says the priors are the same for the Y3 mock analysis and the Y1 re-analysis, but I can't find a place in the text that justifies the prior choices -- did I miss it?}\tianqing{The prior on the nuisance parameters are now different, the priors on cosmological and astrophysical parameters are the same. } 

% I think this justification isn't needed because we comment on this later.  
%\rachel{Justification of this choice?}\tianqing{I left a very unsatisfying justification. Maybe non-PSF should be better-understood?} \rachel{The text gives a practical reason to do this, but it's not an actual justification that explains why this is scientifically valid.  Here's an attempt at that justification: Maybe we could point back to the analysis of the Y3 galaxy-star and star-star correlations, which showed that using PSF vs.\ non-PSF stars gave different $\beta$ values but nearly the same estimate of the shear contamination?   If so, then that motivates just choosing whichever gives you better SNR.} 

%\rachel{I think, to start out the discussion, you need to comment on the bias in the no-systematics model, since we compare everything else to it.  Might be worth citing the Krause et al paper regarding projection effects in high-dimensional analyses inducing small offsets from the true parameters.}\tianqing{I couldn't find that paper, only saw a paper of her about projection effect in the SZ effect. I have explained this in words though, which is similar to how we explained this in the n(z) paper.} \rachel{An example is right before the start of section IV subsection A in https://arxiv.org/pdf/2105.13545.pdf -- I think it's worth citing this paper as well, because it shows this is a uniquitous and understood effect rather than just our speculation on something seen in our analysis.}\tianqing{OK, I have changed the explanation and added the reference. }

%\rachel{Honestly, I don't believe results about errorbars at the level of 5\% are necessarily significant (not sure the chains are stable at that level) or important for making decisions, i.e., I'm not sure I believe we should make choices based on $\pm 5$\% differences. I would suggest replacing this entire paragraph with a statement that the choice between the models shown here only affect the errorbars at the few-percent level, so this is not a significant factor in choosing between these models.}\tianqing{Yeah, concluding anything without an errorbar is risky, I think your version is safer.}

%\rachel{I think the inclusion of PSF vs.\ non-PSF samples is important and should be referenced below.  Other surveys do this, so it's not HSC specific.}\tianqing{Done}

%\rachel{I suggest using an actual enumerate environment on this so that you can change how you break up the list without having to manually change the numbers on the list.  Make latex do the work. :)  Maybe also consider breaking up some of the larger steps.}\tianqing{Done, it still looks very complicated}




%\rachel{Was the 8\% quoted above before or after this cut?  The narrative makes it quite unclear how that number relates to this additional cut.  I would suggest moving any statement of the total size of the non-PSF star sample to after all cuts have been described.}\tianqing{Sorry, the $8\%$ is before the SNR cut, I put that sentence at the end now, and the fraction is corrected to $6\%$ (after the SNR cut)}

 %\rachel{I don't understand the purpose of this sentence.  It sounds like you are trying to blame the differences in the various histograms on sample property differences (difference criteria), which casts doubt on our explanation that we have put forward (i.e., we later propose that the difference is due to over-fitting, which is only a viable explanation if sample property differences are {\em not} responsible).  What is the purpose of doing that?  What evidence do we have that the sample selection differences are responsible, rather than over-fitting?}\tianqing{Right, because the PSF-PSF correlation between the true moments are the same for PSF versus non-PSF. So this statement is vastly overstated. I will delete it. }















